When Explanations Lie: Why Many Modified BP Attributions Fail

Attribution methods aim to explain a neural network's prediction by highlighting the most relevant image areas. A popular approach is to backpropagate (BP) a custom relevance score using modified rules, rather than the gradient. We analyze an extensive set of modified BP methods: Deep Taylor Decomposition, Layer-wise Relevance Propagation (LRP), Excitation BP, PatternAttribution, DeepLIFT, Deconv, RectGrad, and Guided BP. We find empirically that the explanations of all mentioned methods, except for DeepLIFT, are independent of the parameters of later layers. We provide theoretical insights for this surprising behavior and also analyze why DeepLIFT does not suffer from this limitation. Empirically, we measure how information of later layers is ignored by using our new metric, cosine similarity convergence (CSC). The paper provides a framework to assess the faithfulness of new and existing modified BP methods theoretically and empirically. For code see: https://github.com/berleon/when-explanations-lie

==> Makefile <==

NAME = when_explanations_lie
MAIN_TEX = main.tex


.PHONY: arxiv copy compile_arxiv ga_compress build anonymous_code
arxiv: copy compress_figures compile_arxiv


copy:
	rm -rf releases
	mkdir -p releases/build
	cp -r *.tex  \
		*.sty \
		*.bib \
		*.bst \
		figures/ \
		export_defs/ \
		releases/build/
	rm  releases/build/backup.tex

anonymous_code:
	rm -rf anonymous_code
	mkdir -p anonymous_code
	cp -r *.tex  \
		*.sty \
		*.bib \
		*.bst \
		figures/ \
		export_defs/ \
		anonymous_code
	rm  anonymous_code/backup.tex
	sed -i '/icmlauthor/s/.*//' anonymous_code/main.tex
	sed -i '/icmlcorrespondingauthor/s/.*//' anonymous_code/main.tex
	sed -i '/icmlaffiliation/s/.*//' anonymous_code/main.tex
	sed -i '/deletelineforcodesubmission/s/.*//' anonymous_code/main.tex
	ack Leon anonymous_code
	cd anonymous_code && zip -q -r /tmp/latexsource.zip *

compile_arxiv:
	cd releases/build && \
		latexmk -pv  -pdf $(MAIN_TEX) && \
		tar -zcvf ../$(NAME)_arxiv.tar.gz .
	cp releases/$(NAME)_arxiv.tar.gz /tmp

cut-pdf:
	mkdir -p /tmp/wel-camera-ready/
	pdftk releases/build/main.pdf cat 1-12 output /tmp/wel-camera-ready/paper.pdf
	pdftk releases/build/main.pdf cat 13-end output /tmp/wel-camera-ready/supp.pdf

compress_figures:
	chmod +x ./compress_figures.sh
	./compress_figures.sh releases/build/figures

build/$(NAME).pdf: $(MAIN_TEX) figures
	mkdir -p build
	latexmk -pvc  -pdf -jobname=build/$(NAME) $(MAIN_TEX)


supplementary:
	rm -rf /tmp/$(NAME)_pages
	mkdir -p /tmp/$(NAME)_pages
	pdfseparate -f 12 -l 18 build/$(NAME).pdf /tmp/$(NAME)_pages/page_%d.pdf
	pdfunite /tmp/$(NAME)_pages/*  /tmp/supplementary.pdf

pdf2png:
	rm -rf pdftopng
	mkdir -p pdftopng
	cd pdftopng && pdftoppm -png -r 600 ../build/$(NAME).pdf $(NAME)

